EMO-SUPERB: An In-depth Look at Speech Emotion Recognition

Speech emotion recognition (SER) is a pivotal technology for human-computer interaction systems. However, 80.77% of SER papers yield results that cannot be reproduced. We develop EMO-SUPERB, short for EMOtion Speech Universal PERformance Benchmark, which aims to enhance open-source initiatives for SER. EMO-SUPERB includes a user-friendly codebase to leverage 15 state-of-the-art speech self-supervised learning models (SSLMs) for exhaustive evaluation across six open-source SER datasets. EMO-SUPERB streamlines result sharing via an online leaderboard, fostering collaboration within a community-driven benchmark and thereby enhancing the development of SER. On average, 2.58% of annotations are annotated using natural language. SER relies on classification models and is unable to process natural languages, leading to the discarding of these valuable annotations. We prompt ChatGPT to mimic annotators, comprehend natural language annotations, and subsequently re-label the data. By utilizing labels generated by ChatGPT, we consistently achieve an average relative gain of 3.08% across all settings.

==> sections/5.2_Results_of_gap_between_SOTA.tex <==

\begin{table}[]
\fontsize{7}{9}\selectfont
\centering
\caption{The table presents macro-F1 scores of the SER SOTA (denoted ``SOTA'') and the best results from our platform (denoted ``Ours''). The absolute difference is calculated by ours results minus the SOTA results. The \textbf{Model} denotes the best SSLM of our settings.}
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Dataset}    & \textbf{SOTA}  & \textbf{Ours}  & \textbf{Absolute Difference} & \textbf{Model}             \\ \midrule
\textbf{IMPROV (P)} & 0.635          & 0.559          & -7.65\%                      & WavLM                      \\
\textbf{CREMA-D}    & 0.626          & 0.676          & 5.02\%                       & XLS-R-1B                   \\
\textbf{POD(P)}     & 0.360          & 0.350          & -0.93\%                      & WavLM                      \\
\textbf{B-POD (P)}  & 0.273          & 0.266          & -0.66\%                      & XLS-R-1B                   \\
\textbf{IEMOCAP}    & 0.426          & 0.339          & -8.72\%                      & \multicolumn{1}{l}{W2V2 R} \\
\textbf{NNIME}      & 0.220          & 0.209          & -1.10\%                      & WavLM                      \\
\textbf{IMPROV (S)} & 0.336          & 0.433          & 9.68\%                       & \multicolumn{1}{l}{W2V2 R} \\
\textbf{POD (S)}    & 0.259          & 0.384          & 12.46\%                      & XLS-R-1B                   \\
\textbf{B-POD (S)}  & 0.194          & 0.283          & 8.86\%                       & XLS-R-1B                   \\ \midrule
\textbf{Average}    & \textbf{0.370} & \textbf{0.389} & 1.89\%                       & \multicolumn{1}{l}{}       \\ \bottomrule
\end{tabular}
\label{tab:sota}
\end{table}

\subsection{Results of Gap between SER SOTA}
We are interested in the performance gap between the state-of-the-art (SOTA) SER framework and ours, so we conduct the experiences using the SOTA SER proposed by \citep{Wagner_2023} fine-tuning the ``Wav2Vec2-Large-Robust''. Table \ref{tab:sota} summarizes macro-F1 scores of the SER SOTA (denoted ```SOTA'''') and the best results from our platform (denoted ```Ours''''). Surprisingly, the average performance is not that big of a difference, and we got better performance on the CREMA-D, IMPROV (S), POD (S), and B-POD (S). Besides, our method only costs around 24 GPU memory during training, but the SOTA SER model needs more than 34 GPU memory. The proposed method is competitive but more efficient than the SOTA SER model.




==> sections/backup/RQ1.tex <==


\begin{table}[t]
\fontsize{7}{9}\selectfont
\centering
\caption{The table summarizes macro-F1 scores on the IEMOCAP emotion database trained with labels aggregated by MR, PR, and AR.}
\begin{tabular}{@{}crrrr@{}}
\toprule
Dataset          & Ratio   & Total  & Single & Multiple \\ \midrule
IEMOCAP     & 8.23\%  & 32,526  & 29,849         & 2,677            \\
NNIME       & 27.70\% & 25,768  & 18,631         & 7,137            \\
IMPROV (S)   & 49.60\% & 61,702  & 31,096         & 30,606           \\
PODCAST (S)  & 61.69\% & 853,302 & 326,880        & 526,422          \\
B-PODCAST (S) & 74.58\% & 233,284 & 59,310         & 173,974          \\ \bottomrule
\end{tabular}
\label{tab:statics_multilabel}
\end{table}

\begin{table}[h]
\fontsize{7}{9}\selectfont
\centering
\caption{The table summarizes macro-F1 scores when training and testing with each aggregation method for each database. We highlight in bold the best performance for each condition.}
\begin{tabular}{@{}c|c|lll@{}}
\toprule
Upstram                     & Train\textbackslash{}Test & \multicolumn{1}{c}{AR\_Test} & \multicolumn{1}{c}{MR\_Test} & \multicolumn{1}{c}{PR\_Test} \\ \midrule
\multirow{3}{*}{Hubert}     & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{WavLM}      & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{Data2Vec-A} & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{W2v2 R}     & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{DeCoar2}    & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{W2v2}       & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{APC}        & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{VQ-APC}     & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{TERA}       & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{W2V}        & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{Mockingjay} & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{VQ-APC}     & AR\_Train                 & \multicolumn{1}{c}{0.312}    & \multicolumn{1}{c}{0.201}    & \multicolumn{1}{c}{0.199}    \\
                            & MR\_Train                 & \multicolumn{1}{c}{0.299}    & \multicolumn{1}{c}{0.205}    & \multicolumn{1}{c}{0.201}    \\
                            & PR\_Train                 & \multicolumn{1}{c}{0.302}    & \multicolumn{1}{c}{0.205}    & \multicolumn{1}{c}{0.203}    \\ \midrule
\multirow{3}{*}{NPC}        & AR\_Train                 & \multicolumn{1}{c}{0.303}    & \multicolumn{1}{c}{0.197}    & \multicolumn{1}{c}{0.193}    \\ 
                            & MR\_Train                 & \multicolumn{1}{c}{0.284}    & \multicolumn{1}{c}{0.189}    & \multicolumn{1}{c}{0.185}    \\
                            & PR\_Train                 & \multicolumn{1}{c}{0.283}    & \multicolumn{1}{c}{0.188}    & \multicolumn{1}{c}{0.184}    \\ \midrule
\multirow{3}{*}{M CPC}      & AR\_Train                 &                              &                              &                              \\ 
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{PASE+}      & AR\_Train                 &                              &                              &                              \\
                            & MR\_Train                 &                              &                              &                              \\
                            & PR\_Train                 &                              &                              &                              \\ \midrule
\multirow{3}{*}{FBNAK}      & AR\_Train                 & \multicolumn{1}{c}{0.242}    & \multicolumn{1}{c}{0.141}    & \multicolumn{1}{c}{0.140}    \\
                            & MR\_Train                 & \multicolumn{1}{c}{0.234}    & \multicolumn{1}{c}{0.137}    & \multicolumn{1}{c}{0.136}    \\
                            & PR\_Train                 & \multicolumn{1}{c}{0.234}    & \multicolumn{1}{c}{0.137}    & \multicolumn{1}{c}{0.136}    \\ \cmidrule(l){1-5} 
\end{tabular}
\label{tab:multi_label}
\end{table}



\section{RQ1: Rethinking the definition of SER task}
\textbf{Should we regard the SER task as a multi-label recognition task, and does it perform better than the traditional single-label ones?}  
The semantics space theory \cite{Cowen_2021} concluded that emotions are blended and overlap, and we list the statics if the annotators can choose more than one emotion during the labeling process in Table \ref{tab:statics_multilabel}. 
The more recent and extensive databases have higher ratios for selecting multiple emotions (up to 74.58\% in Table \ref{tab:statics_multilabel}). 


However, whether the multi-label SER systems perform better than the single-label systems has not been investigated. 
We conduct two qualitative ways to investigate the questions, frozen and fine-tune SSLMs mentioned in section \ref{ss:framework}.

We prepare the train, development, and test sets in traditional and the new ways. 
The traditional ways to aggregate labels have two different types: majority rule (\textbf{MR}) and plurality rule (\textbf{PR}) and the new way uses all-inclusive rule (\textbf{AR}).
The different aggregation rules causes the different data loss shown in Table \ref{tab:data_loss}.
The MR and PR cause 44.51\% and 18.40\% data loss in average of 9 conditions across six emotion databases, respectively, which also means the test data are not completed. Instead, the AR has no data loss, and few SER studies reveal the performances on the complete test data.

We select the most well-known IEMOCAP corpus to compare the performances among the SER systems trained with three aggregation ways. We use frozen SSLMs way to train and evaluate the SER models. Table \ref{tab:multi_label} summarizes overall the macro-F1 scores of the SSLMs-based SER systems trained with the train sets selected by majority rule (MR, denoted as MR$_{train}$), plurality rule (PR, denote as PR$_{train}$), and all-inclusive rule (AR, denote as AR$_{train}$) evaluate on the test sets obtained by MR (MR$_{test}$), PR (PR$_{test}$), and AR (AR$_{test}$). {\color{blue} Conclusions}

\begin{table}[]
\fontsize{7}{9}\selectfont
\centering
\caption{The table summarizes data loss ratios decided by MR, PR, and AR aggregation methods.}
\begin{tabular}{@{}cccc@{}}
\toprule
Database      & MR      & PR      & AR     \\ \midrule
IEMOCAP       & 31.37\% & 25.32\% & 0.00\% \\
CREMA-D       & 35.80\% & 8.55\%  & 0.00\% \\
IMPROV (P)    & 9.18\%  & 5.63\%  & 0.00\% \\
IMPROV (S)    & 54.18\% & 12.32\% & 0.00\% \\
PODCAST (P)   & 44.81\% & 19.85\% & 0.00\% \\
PODCAST (S)   & 92.01\% & 33.72\% & 0.00\% \\
NNIME         & 25.30\% & 17.16\% & 0.00\% \\
B-PODCAST (P) & 20.25\% & 0.06\%  & 0.00\% \\
B-PODCAST (S) & 87.72\% & 43.02\% & 0.00\% \\ \midrule
Average       & 44.51\% & 18.40\% & 0.00\% \\ \bottomrule
\end{tabular}
\label{tab:data_loss}
\end{table}




\subsection{Related Work}
There still needs to be consensus on generating labels and definitions of emotion recognition tasks. The three most common ways are:  

\begin{itemize}
    \item \textbf{Single-label}: It assumes that each data only can map to one emotion, and this idea is mainly affected by the basic emotion theory \cite{Ekman_1999}. However, it is a comment to observe disagreement between annotators on the one sample, so most SER researchers use majority or plurality rule \cite{Lotfian_2017,Li_2022} to generate one consensus emotion as the learning target. They dropped the data samples that had no consensus emotion class.
    
    \item \textbf{Multi-label}: It assumes that each data could have more than one emotion perception. The multi-label (multiple-hot label) is mainly used in text emotion recognition \cite{Fei_2020}. They take all emotion classes as target emotions even if only one annotator chooses that emotion on the one sample. 
    
    \item \textbf{Distribution-label}: It is assumed that emotion perception is distribution-like and more than one emotion. The distribution label is mainly used in facial expression emotion recognition \citet{Li_2019_5,Xu_2020}. They calculate the distribution based on number of votes for each emotion.
\end{itemize}







==> sections/backup/RQ2.tex <==
\begin{table*}[]
\fontsize{7}{9}\selectfont
\centering
\caption{The table summarizes overall information of the 6 public emotion databases.}
\begin{tabular}{@{\hspace{0.2cm}}c|@{\hspace{0.1cm}}c|@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}}
\toprule
\textbf{Upstream}   & \textbf{Avg.}  & \textbf{IMPROV (P)} & \textbf{CREMA-D} & \textbf{PODCAST (P)} & \textbf{B-PODCAST (P)} & \textbf{IEMOCAP} & \textbf{NNIME} & \textbf{IMPROV (S)} & \textbf{PODCAST (S)} & \textbf{B-PODCAST (S)} \\ \midrule
\textbf{Hubert}     & \textbf{0.385} & 0.553               & 0.675            & 0.342                & 0.262                  & \textbf{0.337}   & 0.197          & 0.427               & \textbf{0.395}       & 0.274                  \\
\textbf{XLS-R-1B}   & 0.384          & 0.552               & \textbf{0.676}   & 0.331                & \textbf{0.266}         & 0.329            & 0.209          & 0.422               & 0.384                & \textbf{0.283}         \\
\textbf{WavLM}      & 0.383          & \textbf{0.559}      & 0.673            & \textbf{0.350}       & 0.252                  & 0.336            & \textbf{0.209} & \textbf{0.430}      & 0.369                & 0.272                  \\
\textbf{Data2Vec-A} & 0.371          & 0.536               & 0.659            & 0.329                & 0.252                  & 0.321            & 0.188          & 0.414               & 0.378                & 0.266                  \\
\textbf{W2V2   R}   & 0.364          & 0.530               & 0.647            & 0.331                & 0.251                  & 0.316            & 0.180          & 0.397               & 0.363                & 0.262                  \\
\textbf{DeCoAR 2}   & 0.362          & 0.512               & 0.646            & 0.308                & 0.256                  & 0.320            & 0.187          & 0.405               & 0.353                & 0.274                  \\
\textbf{W2V2}       & 0.359          & 0.469               & 0.669            & 0.321                & 0.255                  & 0.306            & 0.178          & 0.396               & 0.353                & 0.281                  \\
\textbf{APC}        & 0.349          & 0.497               & 0.608            & 0.298                & 0.249                  & 0.316            & 0.186          & 0.389               & 0.340                & 0.261                  \\
\textbf{VQ-APC}     & 0.346          & 0.497               & 0.603            & 0.296                & 0.246                  & 0.312            & 0.181          & 0.389               & 0.331                & 0.261                  \\
\textbf{TERA}       & 0.344          & 0.493               & 0.596            & 0.295                & 0.240                  & 0.308            & 0.193          & 0.385               & 0.337                & 0.253                  \\
\textbf{W2V}        & 0.342          & 0.448               & 0.612            & 0.300                & 0.246                  & 0.304            & 0.188          & 0.387               & 0.336                & 0.258                  \\
\textbf{Mockingjay} & 0.335          & 0.485               & 0.570            & 0.275                & 0.244                  & 0.307            & 0.185          & 0.379               & 0.318                & 0.253                  \\
\textbf{VQ-W2V}     & 0.331          & 0.442               & 0.605            & 0.292                & 0.246                  & 0.294            & 0.156          & 0.361               & 0.325                & 0.260                  \\
\textbf{NPC}        & 0.331          & 0.470               & 0.570            & 0.274                & 0.240                  & 0.301            & 0.172          & 0.362               & 0.333                & 0.256                  \\
\textbf{M CPC}      & 0.317          & 0.453               & 0.515            & 0.265                & 0.228                  & 0.285            & 0.175          & 0.337               & 0.318                & 0.281                  \\
\textbf{PASE+}      & 0.317          & 0.456               & 0.521            & 0.274                & 0.233                  & 0.292            & 0.178          & 0.349               & 0.306                & 0.248                  \\ \midrule
\textbf{FBANK}      & 0.191          & 0.305               & 0.144            & 0.186                & 0.199                  & 0.242            & 0.120          & 0.184               & 0.170                & 0.168                  \\ \bottomrule
\end{tabular}
\label{tab:results}
\end{table*}

\section{RQ2: Performances of modern multi-label SER systems}
\textbf{ Which self-surprised learning models are the best candidate for training
multi-label SER systems.} 
Table \ref{tab:results} summarizes 16 SSLMs and hand-craft results. 



\subsection{Layer Anlaysis of SSLMs for SER}
We reveal layer-wise analyses of SSLMs by taking the weights of each layer for six different public emotion databases. 
Also, we demonstrate two conditions for better showing which layers have SER-related information below. 
(1) Do the shallow or deep layers have more information for the SER task within the emotion corpus? 
(2) Within models, what are the differences across 16 SSLMs? Besides, we are interested in whether the SSLMs have enough paralinguistic information to recognize complex emotions, such as frustration.

\subsubsection{Within Corpus, Across SSLMs}

{\color{blue}
To show layer-wise weights
}

\subsubsection{Within SSLMs, Across Corpus}
{\color{blue}
To show layer-wise weights
}



\subsubsection{Related Work}
While the SSLMs-based models achieve state-of-the-art performances across various speech tasks, the interpretations of what SSLMs learned are still unsolved puzzles and more complicated than the handcraft features, such as pitch and intensity. 
One common way is to analyze the weights of layers of SSMs for specific tasks \citep{Pasad_2021,Pasad_2023,Pasad_2023_2} . 
However, few papers conduct the analyses for SER; very recently, \citet{Li_2023} analyzed the wav2vec 2.0 on the IEMOCAP and concluded that the wav2vec 2.0 can not provide paralinguistic information for the SER task and the final layer of the wav2vec 2.0 has the most minor information for SER task. 
However, \citet{Li_2023} applied the following restrictions to select samples of the IEMOCAP--combine excitement into happiness, only focus on four emotions (anger, happiness, sadness, and neutral states), and remove the data samples that have no consensus on one emotion. 
Those restrictions limit the ability to show actual performances and analyses of SER systems.

==> sections/backup/RQ3.tex <==
\begin{table}[]
\fontsize{7}{9}\selectfont
\centering
\caption{The table summarizes performances of the various SSLMS-based SER systems trained with the labels elicited by different modalities.}
\begin{tabular}{@{}c|cccc@{}}
\toprule
\textbf{Upstream}   & \textbf{Audio} & \textbf{Face} & \textbf{Audio-visual} & \textbf{Combination} \\ \midrule
\textbf{XLS-R-1B}   & 0.676          &               &             &              \\
\textbf{WavLM}      & 0.673          & 0.629         & 0.696       & 0.733        \\
\textbf{Hubert}     & 0.675          & 0.615         & 0.682       & 0.721        \\
\textbf{Data2Vec-A} & 0.659          & 0.593         & 0.656       & 0.698        \\
\textbf{W2V2   R}   & 0.648          & 0.560         & 0.613       & 0.674        \\
\textbf{DeCoAR   2} & 0.646          & 0.583         & 0.643       & 0.674        \\
\textbf{W2V2}       & 0.669          &               &             &              \\
\textbf{APC}        & 0.608          & 0.543         & 0.604       & 0.630        \\
\textbf{VQ-APC}     & 0.603          & 0.538         & 0.602       & 0.623        \\
\textbf{TERA}       & 0.596          & 0.542         & 0.604       & 0.623        \\ 
\textbf{W2V}        & 0.612          & 0.539         & 0.605       & 0.635        \\
\textbf{Mockingjay} & 0.570          & 0.534         & 0.578       & 0.605        \\
\textbf{VQ-W2V}     & 0.605          &               &             &              \\
\textbf{NPC}        & 0.570          & 0.527         & 0.582       & 0.603        \\
\textbf{PASE+}      & 0.521          &               &             &              \\
\textbf{M   CPC}    & 0.529          & 0.476         & 0.526       & 0.560        \\
\textbf{FBANK}      & 0.144          & 0.158         & 0.153       & 0.125        \\ \bottomrule
\end{tabular}
\label{tab:cremad_modality_sslms}
\end{table}

\section{RQ3: Impacts of different stimulus modalities on emotion perception}
\label{ss:stimulus}

\textbf{Should we use the datasets annotated using multi-modal information to train and evaluate SER systems} 
Emotion perception could be affected by different stimulus modalities. 

The CREAM-D database \citep{Cao_2014} is the most suitable to investigate the question. 
The database collects annotations by providing different stimulus modalities: face-only (\textbf{Face}), voice-only (\textbf{Voice}), Audio-visual (\textbf{AV}), and combination (\textbf{Combination}). 
We take the annotations elicited by different modalities and calculate the multi-label distribution labels for six emotions. 
We use the concordance correlation coefficient (CCC) to measure the correlation between different conditions shown in Table \ref{tab:cremad_modality_correlation}. 
Surprisingly, the CCC between voice-only and audio-visual ones is only 0.459, but the CCC between face-only and audio-visual ones is 0.805. 
Then, the CCC between audio-only and combination (0.745) is lower than the one between face-only and combination (0.875) and the one between audio-visual and combination (0.913).  

Besides, Table \ref{tab:cremad_modality_sslms} reveal the performance differences of the model trained with the the labels elicited by different modalities. Surprisingly, the performances of SER models (except FBANK) trained with the combination labels have the best performances. The models (except FBANK) trained with the face-only labels have the lowest performances. The labels elicited by different modalities causes different performances of SER systems. We might rethink about choice of the annotations for the SER task.

\subsection{Related Work}



\begin{table}[]
\fontsize{7}{9}\selectfont
\centering
\caption{The table summarizes performances of the various SSLMS-based SER systems trained with the labels elicited by different modalities.}
\begin{tabular}{@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}}
\toprule
\textbf{Stimulus Modality} & \textbf{Face} & \textbf{Voice} & \textbf{Audio-visual} & \textbf{Combination} \\ \midrule
\textbf{Face}                & 1.000         & 0.459          & 0.805                 & 0.875            \\
\textbf{Voice}               & 0.459         & 1.000          & 0.573                 & 0.745            \\
\textbf{Audio-visual}        & 0.805         & 0.573          & 1.000                 & 0.913            \\
\textbf{Combination}             & 0.875         & 0.745          & 0.913                 & 1.000            \\ \bottomrule
\end{tabular}
\label{tab:cremad_modality_correlation}
\end{table}





==> sections/backup/RQ4.tex <==
\section{RQ4: Typed descriptions of emotion perception}
\textbf{How to utilize the typed descriptions to improve multi-label SER performances with the GPT's assistance?} We take the eight-class primary emotion as the target emotions and use the typed descriptions to improve the SER systems. Our approach is to design a prompt to ask GPT-4 Turbo (``gpt-4-0125-preview'') \citep{Achiam_2023} to adjust the 8-dimensional distribution-like labels. The goal of prompt is to ask GPT-4 as a knowledgeable assistant psychologist. Its role is to analyse the given distribution of the target emotions and typed descriptions from annotators and then adjust the distribution. The completed prompt is in Appendix section \ref{ss:prompt}. {\color{blue} Table \ref{tab:GPTs} summarizes the macro-F1 scores on the MSP-PODCAST (P). The labels generated by the GPTs can improve the SER performances.
}




\begin{table}[]
\fontsize{7}{9}\selectfont
\centering
\caption{The table summarizes macro-F1 scores of CREMA-D and SAIL-IEMOCAP emotion databases in different scenarios.}
\begin{tabular}{@{}ccc@{}}
\toprule
Upstream   & Standard & With GPTs \\ \midrule
Huber      & 0.342    & 0.350     \\
XLS-R-1B   & 0.331    &           \\
WavLM      & 0.350    &           \\
Data2Vec-A & 0.329    &           \\
W2V2   R   & 0.331    & 0.335     \\
DeCoAR     & 0.308    &           \\
W2V2       & 0.321    &           \\
APC        & 0.298    & 0.307     \\
VQ-APC     & 0.296    & 0.310     \\
TERA       & 0.295    & 0.306     \\
W2V        & 0.300    & 0.305     \\
Mockingjay & 0.275    & 0.298     \\
VQ-W2V     & 0.292    & 0.299     \\
NPC        & 0.274    & 0.290     \\
M   CPC    & 0.265    & 0.290     \\
PASE+      & 0.274    &           \\
FBANK      & 0.186    & 0.186     \\ \bottomrule
\end{tabular}
\label{tab:GPTs}
\end{table}

\subsection{Related Work}
The most related work is the study \citep{Chou_2022}. They extracted the typed descriptions and correct the typo, and normalized the part-of-speech to match the words in the positive and negative dictionaries \emph{linguistic inquiry and word count} (LIWC) 2015 toolkit (LIWC 2015) \citep{Pennebaker_2015}. They mapped the words that are not in the dictionaries into the ambiguous class. Then, they calculate the 3-dimensional vector (negative, ambiguous, positive) for another task. They found the task can improve recognition power of target emotions by using multi-task learning. Different from them, we do not do any preprocessing on the typed words and take them as input for GPT-4 to adjust the target distribution-like labels.

==> sections/backup/experimental.tex <==
\section{Experimental Setup}
We first introduce our experimental settings to investigate the research questions above, including database and pre-processing, models, training, and evaluation procedures. Our north star is to reveal the actual performances of SER systems with the suitable definition of SER task, multi-label SER task. 

We collect almost all the public pre-trained SSLM models and use the SUPERB way to train and evaluate the SER systems with the new type of labels. 
We show the 16 SSLMs' SER performances evaluated across six public emotion databases in English and Chinese in 9 conditions. 
We also show the correlation analyses between layers and SER tasks for 16 SSLMs and two hand-craft feature sets. 
In addition, we provide our insights to select the benchmark database for the SER task with experimental results.





\subsection{Resources}
We include six different public emotion databases to show the SER performances of SSLMs-based based on the data samples that have yet to be revealed. 
We maximize the usage of the emotional annotations and use pre-defined emotion options as target emotions. We exclude the ``Other" used in some databases to allow the annotators to type their emotional descriptions by words or sentences. Yet, we propose an way to  typed descriptions to improve the performances of SER systems.  
Table \ref{tab:databases} in Appendix summarizes detailed information about six emotion databases. The details about the databases are as follows.

\subsubsection{The SAIL-IEMOCAP}
The SAIL-IEMOCAP \citep{Busso_2008_5}, referred here to as \textbf{IEMOCAP}, collects motion capture, audio, and video recordings from five dyadic conversations acted by ten professional actors in English. 
Each session has one female and one male speaker, and the session setting is lovers-in-relationship interactions. 
The database setting consists of scripted and spontaneous spoken conversations. 
The actors are provided with selected scripts to elicit emotions. 
The recorded sessions were manually segmented into 100,39 utterances and transcribed. 
Then, the utterances were played in order for annotators to choose emotions from given options containing ten emotions (neutral, happiness, sadness, anger, surprise, fear, disgust, frustration, excitement, and “other”) and blank space for leaving emotional descriptions, referred as typed descriptions. 
All annotators can choose more than one emotion during the labeling process, and each utterance has at least three annotators. 
There are 12 unique annotators; half are actors, and the left is naive annotators. 
The perceptual annotations are from self-perception and observed perception, one of the major differences from another emotion database. 
To avoid the difficulty of reproducibility concluded in \citep{Antoniou_2023}, we provide details of split sets in Appendix \ref{sss:cviemocap} since the corpus did not provide standard split sets.

\subsubsection{The CREAMA-D}
The CREMA-D \citep{Cao_2014} contains high-quality audio-visual clips from 91 professional actors. 
There are 43 female and 48 male actors. 
All actors were asked to record one of the selected 12 sentences in one of six emotions (anger, disgust, fear, happiness, sadness, and neutral state). 
There are 7,442 clips in English that have 2,443 unique annotators annotated via a crowdsourcing platform. 
Each clip has at least six annotators, and each annotator can choose only one of six emotions for each utterance. 
The process of perceptual annotations has three scenarios: voice-only, face-only, and audio-visual. 
The voice-only setting only provides the voice of clips for annotators to listen to; 
the annotators can only watch the faces of actors in clips without voice sound in the face-only setting; 
the audio-visual setting allows annotators to watch faces and listen to the voices of clips. In this work, we only use emotional annotations in the voice-only setting for SER. 
Most of the prior SER studies used audio-visual setting annotations (or did not provide information) as a learning target. 
However, huge differences exist in perceived emotions elicited by audio-only, face-only, and audio-visual clips and will be discussed in more detail in section \ref{ss:stimulus}. 
We also provide the details of split sets used in the paper described in Appendix \ref{sss:cvcremad}.

\subsubsection{The MSP-IMPROV}
The MSP-IMPROV \citep{Busso_2017}, referred here to as \textbf{IMPROV}, consists of high-quality audio-video sessions acted by 12 actors in English in four emotions (anger, happiness, sadness, and neutral state). 
Every dyadic interaction has one male and one female speaker in four different recording scenarios: preparation, scripted, improvised, and improvised-scripted scenes. 
All sessions are manually segmented into 8,438 clips, each with at least five different annotators through the crowdsourcing platform. 
The MSP-IMPROV utilized the quality control method proposed in \citep{Burmania_2015} to detect and remove the bad annotators. 
The annotation process has two scenarios: primary (\textbf{P}) and secondary (\textbf{S}) emotions. 
The primary only allows annotators to choose one emotion from the five emotions: anger, happiness, sadness, neutral state, and "other." 
Secondary emotions consist of the six primary emotions: frustration, depression, disgust, excitement, fear, and surprise. 
We exclude 53 utterances annotated by "other" from all annotators. 
All annotators are allowed to typed descriptions if they choose ``other'' options.
The database also did not split the standard train, development, and test sets, so we introduce the split sets in Appendix \ref{sss:cvimprov}.

\subsubsection{The MSP-PODCAST}
The MSP-PODCAST \citep{Lotfian_2019_3}, referred here to as \textbf{PODCAST}, collected spontaneous and diverse emotional speech from various real-world podcast recordings with a commercial license. 
All podcast recordings are split into utterances. Afterward, the MSP-PODCAST uses a crowdsourcing platform to collect the annotations and uses the quality checking process in \citep{Burmania_2015} to track the quality of annotators. 
The labeling setting is similar to the MSP-IMPROV, including primary and secondary scenarios. 
The major difference is the number of emotions in the given options. 
The primary emotion (\textbf{P}) has nine options: anger, sadness, happiness, surprise, fear, disgust, contempt, neutral, and ``other'', allowing annotators to typed the words to describe their emotion perception.
Also, the secondary emotion (\textbf{S}) contains the primary emotion and eight more classes: amusement, frustration, depression, concern, disappointment, excitement, confusion, and annoyance (17 options in total). 
Each utterance consists of at least five different annotators. 
We use the release version 1.11 of the database, including 84,030 utterances in the train set, 19,815 in the development set, 30,647 in the test1 set, 14,815 in the test2 set, and 2,347 in the test3 set. 
We combine the test1 and test2 as one test set in the paper, and we exclude the test3 set because it is a hidden private set, which did not provide any annotations for the test3 set. 
There are more than 2,172 unique speakers and 14,363 annotators in total. 

\subsubsection{The BIIC-NNIME}
The BIIC-NNIME \citep{Chou_2017}, referred here to as \textbf{NNIME}, consists of video, audio, and physiology recordings of dyadic conversations acted by 43 actors in Mandarin Chinese. 
All sessions are spontaneous and improvised without scripts in six emotional scenes, including anger, frustration, happiness, sadness, surprise, and neutral states. 
The atmosphere of dyadic interaction is the daily life at home. 
All sessions are manually segmented into 5596 clips. 
We exclude turns annotated by ``other" from all annotators or by less than three annotators. 
The major difference from other emotion datasets is that the corpus annotated speech and non-verbal behaviors, including laughing, sighing, sobbing, and other vocal bursts. 
The database contains 43 unique speakers and six different annotators. 
The labeling process is similar to the SAIL-IEMOCAP.
All annotators watch clips in order and choose emotions from the given 12 emotion options: anger, frustration, disappointment, sadness, fear, surprise, excitement, happiness, relaxation, joy, neutral state, and ``other." 
The corpus allows the annotators to use the words to express their emotion perception in Chinese.
The corpus did not provide standard split sets for training deep-learning models, so we also provide details of split sets in Appendix \ref{sss:cvnnime} since the corpus for reproducibility.


\subsubsection{The BIIC-PODCAST}
The BIIC-PODCAST \citep{Upadhyay_2023}, referred here to as \textbf{B-PODCAST}, is a variant of MSP-PODCAST but in Mandarin Chinese. 
All audio recordings come from real-world podcasts with a commercial license. 
The major difference is the labeling process. 
The corpus did not use a crowdsourcing platform but recruited students from the college as annotators for better quality control. 
The database uses the same quality assessment as the MSP-PODCAST. 
We use the release version 1.01 of the BIIC-PODCAST. 
There are 48815 utterances in the train set, 10845 in the development set, and 10340 in the test set. 
At least five annotators annotate all utterances, and the emotional annotators contain primary emotions (\textbf{P}) and secondary emotions (\textbf{S}) as the same as the MSP-PODCAST. 



\subsection{Preprossessing}
We ensure the existence of audio recordings and extract the audio recordings if the original databases only provide video clips. 
Then, we separate the audio into a monophonic channel if the original data is stereo. 
Also, we resample the audio into 16k Hz if the sample rate is not 16k Hz. 
In Appendix Table \ref{tab:databases}, we conclude with other detailed statics information.
Before passing the speech input, we do normalization them by minus mean and divide the standard deviation of of the training set for all our experiments.

\subsection{Selection Emotion Classes}
Most SER prior studies \citep{Atmaja_2022} only choose anger, happiness, sadness, and neutral state emotions as target emotions. 
In addition, they regard the excitement/joy annotations as happiness; however, excitement and happiness are not the same emotions, and those two emotions are correlations. 
Different from them, we used all original emotion sets (except "Other"), and we did not combine any emotions into another emotion for balancing data (e.g., combine excitement into happiness) to reveal the actual performances and natural distributions to the real conditions. Some databases allow annotators to type their own words to describe their emotion perception if they choose "Other". We introduce an potential way to prompt large language model to combine the emotional information into the target emotions. More details are in section \ref{ss:description}. 

\subsubsection{Label Generation}
\label{ss:label}
To compare the performance differences between single-label and multi-label SER, we use three common aggregation methods to decide the labels for training and evaluate the SER systems.

\begin{itemize}
    \item \textbf{Majority Rule}: It only selects the emotion class that obtains more than half of annotations as target emotion, drops other minority annotations, and removes the data that have no consensus. 
    
    \item \textbf{Plurality Rule}: It selects that emotion class with more annotations as the target emotion and ignores the minority labels and the data without consensus votes.
    
    \item \textbf{All-inclusive Rule}: It takes as many annotations as possible and calculates the distribution-like (soft label) based on the number of each emotion class. It does not leave any samples behind. 

\end{itemize}

The all-inclusive Rule (AR) is first used in \citet{Chou_2022}, and we are motivated by semantics space theory \citep{Cowen_2021} to name the method as AR for better reelecting that emotion perception is high-dimensional, and boundaries of emotions are blended and overlap. We use those three aggregation methods to obtain the labels to train and evaluate the SER systems for comparison. 
For instance, consider a four-class emotion recognition task, and the emotion classes contain neutral, anger, sadness, and happiness. 

Assume we collect five annotations from five different unique raters for one sample, and the annotations contain neutral (N), anger (A), anger (A), sadness (S), and sadness (S). 
With the AR aggregation method, we calculate the label distributions, which for this case is (N, A, S, H) = (0.2, 0.4, 0.4, 0.0) for training SER systems. 
During inference, the threshold is 1/4=0.25, and the ground truth is converted to (0,1,1,0); 
we consider the predictions for three different models: (0.2,0.35,0.35,0.1), (0.1,0.45,0.45,0.0), and (0.45,0.1,0.0,0.45). 
The three predictions are transformed into (0,1,1,0), (0,1,1,0), and (1,0,0,1), respectively, using the threshold. 
In these cases, only the first two predictions are fully corrected. In terms of MR and PR methods, however, they drop the sample.
We also use the label smoothing strategy proposed by Szegedy et al. \cite{Szegedy_2016} to smooth the vector using the smoothing parameter 0.05, where a small probability is given to emotional classes with zero value. The label smoothing strategy is also used for the single one-hot vector. 

\subsubsection{Utilization of Typed Descriptions}
\label{ss:description}
The PODCAST, IEMOCAP, NNIME, and IMPROV allows annotators to use their own words/sentences to describe the emotion perception corresponding to the stimulus data. We take the PODCAST to validate whether our propose method can improve the emotion perceptions, and we the typed descriptions of the PODCAST in Figure \ref{fig:wordcloud}. 

\begin{figure}[b]
\centering
\includegraphics[width=0.9\linewidth]{sections/word_cloud.pdf}
\vspace{-0.3cm}
\caption{The figures shows typed descriptions of the MSP-PODCAST for an example.} 
\label{fig:wordcloud}
\end{figure}


\subsection{Models Training and Evaluation}
We use the Adam optimizer \cite{Kingma_2014_2} with a 0.0001 learning rate. We group 32 utterances to construct each mini-batch and update the model for 100 epochs.

\subsubsection{Class-balanced Objective Function}
We use the class-balanced cross-entropy loss as our primary objective function since the annotation distributions of all used databases are imbalanced shown in Appendix Table \ref{tab:databases}. However, most SER studies have not considered the issue, so we integrate the ``class-balanced cross-entropy loss'', referred as \textbf{CBCE}, in the study of Cui \citep{Cui_2019}, but we did not conduct other existing class-balance objective functions. The main idea is to add a weighting factor to adjust the values of the used loss function based on the inverses of the class frequency considering the training set. The factor is $ \frac{1-\beta}{1-\beta^{n_{j}}} $, where $n_{j}$ is the number of positive samples in the $j^{th}$ emotion class in the train set, and $\beta \in (0,1]$ is a hyperparameter. The number of factors to weigh the loss values equals to the number of target emotions. The CBCE value can be calculated using Eq. \ref{eq:cbl}, where $\mathcal{L_{\mathit{CE}}}^{(j)}$ is the value of cross-entropy loss for the $j^{th}$ emotion.


\begin{align} 
\mathcal{L_{\mathit{CBL}}} &=  \sum_{j=1}^{K} ( \frac{1-\beta}{1-\beta^{n_{j}}}  \cdot \mathcal{L_{\mathit{CE}}}^{(j)}). 
\label{eq:cbl}
\end{align}



\subsubsection{Standard Split Set Preparation}
The IEMOCAP, CREMA-D, IMPROV, PODCAST, and NNIME did not provide standard training, development, and test splits. Most SER studies \citep{Atmaja_2022} use their way to split the sets. The authors should have provided details about how they split development. Most of them only provided details about how they split training and test sets. The missing information causes the difficulty of reproducibility, and \citet{Antoniou_2023} also points out the issue on the IEMOCAP corpus. We provide the details of how we split the train, development, and test sets in Appendix section \ref{ssec:cv} to close the reproducibility gap.




\subsubsection{Evaluation Metrics}
We use the macro-F1 scores to evaluate the SER performance, simultaneously considering recall and precision rates. 
Additionally, we show the performances of multi-label SER systems trained with the all-inclusive that maximize the usage of all emotional annotations, and the macro-F1 supports the evaluation of multi-label classification. 
Also, the distributions of emotion classes in the six emotion databases are imbalanced, so Using macro-F1 scores is more desirable than weighed-F1 or micro-F1 scores,
In terms of distribution-like  multi-label as the training target, and the target classes are selected by applying thresholds over the ground truth. 
We consider a prediction a success if the proportion for a class is above $1/C$, where $C$ is the number of emotional classes, following the approach adopted by previous studies \cite{Riera_2019,Chou_2022} mentioned in section \ref{ss:label} for measure macro-F1 scroes. 


\subsection{SER Framewrok}
\label{ss:framework}
We mainly use two different ways to train and evaluate the SER systmes, frozen SSLMS and fine-tuned SSLMs, trained with labels aggregated by three different rules, MR, PR, and AR. 

\subsubsection{Frozen SSLMs}
We use the same setting of the downstream models on emotion recognition (ER) in the SUPERB \citep{Yang_2021} for fair comparison. 
We add an attention linear layer on each layer of SSLMs and use the mean-pooling linear layer for utterance-level SER tasks training with the cross-entropy objective function. 
The number of nodes before the prediction layer is 256.
We collect 16 public SSLMs and follow the review study \citep{Mohamed_2022} definition to classify the SSLMs into three types as follows. 
There exists many variants for some SSLMs such Wav2vec2 larger or base. We select the largest size of SSLMs for each variant representation, but we only use wav2vec2 XLS-R (1b) (not 2b) because the limits of computational resources.
We also list the additional class, hand-crafted features, for comparsions. 



\begin{itemize}
    \item \textbf{Generative models}: PASE+ \citep{Ravanelli_2019}, APC \citep{Chung_2019}, Mockingjay \citep{Liu_2020}, TERA \citep{Liu_2021}, NPC \citep{Liu_2021_2}, DeCOAR 2.0 \citep{Ling_2020}, VQ-APC \citep{Chung_2020}
    
    \item \textbf{Constrictive models}: VQ-Wav2Vec \citep{Baevski_2020_2}, modified CPC \citep{Rivière_2020}, Wav2Vec \citep{Schneider_2019}, Wav2Vec2 \citep{Baevski_2020}, Wav2vec2 Robust \citep{Hsu_2021_2}, Wav2Vec2-XLS-R \citep{Babu_2021}

    \item \textbf{Predictive models}: HuBERT \citep{Hsu_2021}, Data2Vec (Audio), \citep{Baevski_2022}, WavLM \citep{Chen_2022}
    
    
    \item \textbf{Hand-craft features}: FBANK (log mel filterbank) and openSMILE (low-level descriptors, ComParE 2016 feature set) \citep{Eyben_2010}.
\end{itemize}




\subsubsection{Fine-tune SSLMs}

We are interested in performance differences between fine-tuned and frozen SSLMs, so we use one of the used SER frameworks in the \citep{Wagner_2023}, which fine-tuned the pre-trained  ``wav2vec2-large-robust'' model proposed in \cite{Hsu_2021}. We follow the study \citep{Wagner_2023} to remove the 12 transformer layers from the top of the 24 transformer layers used in this architecture, which is shown to preserve the recognition performance with fewer parameters. The study \citep{Wagner_2023} attached two hidden layers and the softmax output layer on top of the ``wav2vec2-large-robust'' model, where each hidden layer has 1,024 nodes. They are implemented with the \emph{rectified linear unit} (ReLU) activation function. The study \citep{Wagner_2023} aggregated the outputs of the model by using average pooling per utterance, then feeding it to the classification layers, and the dropout function used $p=0.5$ to the first and second layers of the classification layers to regularize the model. 



